Quantum Amnesia Leaves Cryptographic Mementos: A Note On Quantum Skepticism

Leonard Shelby, the protagonist of Memento, uses mementos in the form of tattoos and pictures to handle his amnesia. Similar to Leonard, contemporary quantum computers suffer from "quantum amnesia": the inability to store quantum registers for a long duration. Quantum computers can only retain classical "mementos" of quantum registers by measuring them before those vanish. Some quantum skeptics argue that this quantum amnesia is inherent. We point out that this variant of a skeptic world is roughly described by the quantum bounded storage model, and although it is a computational obstacle that annuls potential quantum computational advantage, the seemingly undesired properties provide a cryptographic advantage. Namely, providing exotic primitives promised by the quantum bounded storage model, such as unconditionally secure commitment and oblivious transfer schemes, with constructions involving nothing but transmission and measurement of BB84 states.

==> macros.tex <==
\RequirePackage{etex}
\ifnum\toc=1 
    \usepackage[nottoc]{tocbibind} %This adds the bibliography to the table of contents (of course, only if it exists). There is no need to add the table of contents page to the table of contents, hence the option "nottoc".
\fi
\ifnum\sigconf=0\usepackage{authblk}\fi \usepackage{silence} %authbulk must loaded before the silence package!!
\usepackage[modulo]{lineno}
\usepackage{amsthm,amssymb,amsfonts,latexsym,color,paralist,url,ifdraft,mathrsfs,thm-restate,comment,bbold,booktabs,wrapfig}

\usepackage{footnote}%for savenotes environment

\usepackage[utf8]{inputenc} \usepackage[autostyle=false, style=english]{csquotes} \MakeOuterQuote{"}

%csquotes after inputenc
\usepackage[T1]{fontenc}
\ifnum\sigconf=0
    \ifnum \shownomenclature=1
        \usepackage[refpage,prefix]{nomencl}
        \newcommand*{\nom}[3]{#2\nomenclature[#1]{#2}{#3}} 
        \makenomenclature
        % the following part makes the nomenclature to be a section rather than a section*. It also gives it a label. In the beginning, I had a solution which was based on the following url, but it stopped working, and that's why it is commented out: https://tex.stackexchange.com/questions/124608/how-to-format-the-name-of-a-nomenclature
        %\xpatchcmd{\thenomenclature}{
        %\section*{\nomname}}{% Replace it by the following
        %\section{\nomname}\label{sec:nomenclature}
        %}{\typeout{Success!}}{\typeout{Failure}}
        
        %since the previous solution didn't work, we simply redefine the command itself. See here for the original command: https://github.com/borisveytsman/nomencl/blob/master/nomencl.dtx
  \makeatletter
        \def\thenomenclature{%
  \providecommand*{\listofnlsname}{\nomname}%
  
    
      \section{\nomname}
      \label{sec:nomenclature}    
      \if@intoc\addcontentsline{toc}{section}{\nomname}\fi%
    
  
  \nompreamble
  \if@nomentbl
    \let\itemOrig=\item
    \def\item{\gdef\item{\\}}%
    \expandafter\longtable\expandafter{\@nomtableformat}
  \else
    \list{}{%
      \labelwidth\nom@tempdim
      \leftmargin\labelwidth
      \advance\leftmargin\labelsep
      \itemsep\nomitemsep
      \let\makelabel\nomlabel}%
  \fi
}
\makeatother 
    \fi
    
    \usepackage[draft=false,pageanchor]{hyperref}
    \def\pagedeclaration#1{, \hyperlink{page.#1}{page\nobreakspace#1}} %This is needed for the nomenclature
    \usepackage{doi}

    \usepackage[final]{graphicx}
\fi

 %\usepackage{mathtools} \mathtoolsset{showonlyrefs} %the mathtools way does not work nicely with sigconf. I *think* aotunum works in all cases.
\ifdraft{\usepackage{showlabels}}{} %must be after use package{hyperref}.

%\usepackage[refpage,prefix]{nomencl} \newcommand*{\nom}[2]{#1\nomenclature{#1}{#2}} \makenomenclature
%\usepackage[displaymath,textmath,sections,graphics,floats]{preview}
%\RequirePackage{silence}
\WarningFilter{l3regex}{This package is obsolete }

\usepackage [ lambda,advantage , operators , sets , adversary , landau , probability , notions , logic ,ff, mm,primitives , events , complexity , asymptotics , keys]{cryptocode}
%the following commands are defined by cryptocode. Define these ourselves if needed: \newcommand{\poly}{\mathrm{poly}} \newcommand{\prob}[1]{\Pr[ #1 ]} \newcommand{\norm}[1]{\left\| #1 \right\|} \newcommand{\RR}{\mathbb{R}} \newcommand{\FF}{\mathbb{F}} \newcommand{\CC}{\mathbb{C}} \newcommand{\NN}{\mathbb{N}}\DeclarePairedDelimiter\ceil{\lceil}{\rceil} \DeclarePairedDelimiter\floor{\lfloor}{\rfloor}
\renewcommand{\verify}{\ensuremath{\mathsf{verify}}} 


%\renewcommand{\sfdefault}{phv}
%\renewcommand{\rmdefault}{ptm}

\ifdraft{\newcommand{\authnote}[3]{{\color{#3} {\bf  #1:} #2}}}{\newcommand{\authnote}[3]{}}
\newcommand{\note}[1]{{\color{red}#1}}
%Example for how this should be used, in main file:
%\newcommand{\onote}[1]{\authnote{Or}{#1}{blue}}


\newcommand{\CNOT}{\mathrm{CNOT}}
\newcommand{\defeq}{\stackrel{\mathrm{def}}{=}}

\newcommand{\const}{\mathrm{const}}

\newcommand{\bra}[1]{\langle #1 \vert}
\newcommand{\ket}[1]{\vert #1 \rangle}
\newcommand{\ketbra}[1]{\vert #1 \rangle \langle #1 \vert}
\newcommand{\braket}[2]{\langle #1 \vert #2 \rangle}
\newcommand{\conjugate}[1]{#1^{\dagger}}
\newcommand{\tensor}{\otimes}
\DeclareMathOperator{\tr}{Tr}
\DeclareMathOperator{\Tr}{Tr}
\newcommand{\transpose}[1]{#1^{\mathsf{T}}}
\ifdraft{\linenumbers}{}

\DeclareMathOperator{\spn}{span}
\DeclareMathOperator{\E}{\mathbb{E}}

%\PreviewMacro*\onote
%\PreviewMacro*\nom
%\PreviewMacro*\ifdraft
%\DeclareMathOperator*{\E}{\scalerel*{\mathbb{E}}{\textstyle\sum}}


\newcommand{\ra}[1]{\renewcommand{\arraystretch}{#1}}

%document specific
\usepackage{algorithm,algorithmicx,algpseudocode}
\usepackage[normalem]{ulem}

\newcommand{\BQP}{\textsf{BQP}}

\newcommand{\decrypt}{\ensuremath{\mathsf{decrypt}}}
\newcommand{\encrypt}{\ensuremath{\mathsf{encrypt}}}
\newcommand{\otr}{\ensuremath{\mathsf{OTR}}}
\newcommand{\stamp}{
 {\mathchoice
  {\includegraphics[height=1.8ex]{RubberStamp}}
  {\includegraphics[height=1.8ex]{RubberStamp}}
  {\includegraphics[height=1.2ex]{RubberStamp}}
  {\includegraphics[height=0.9ex]{RubberStamp}}
 }
}
%\newcommand{\keygen}{\ensuremath{\mathsf{key\textit{-}gen}}}
\newcommand{\tokengen}{\ensuremath{\mathsf{token\textit{-}gen}}}
%\newcommand{\sign}{\ensuremath{\mathsf{sign}}}
%\newcommand{\verify}{\ensuremath{\mathsf{verify}}}


\usepackage{tikz}
\usetikzlibrary{arrows,chains,matrix,positioning,scopes}
%
\makeatletter
\tikzset{join/.code=\tikzset{after node path={%
\ifx\tikzchainprevious\pgfutil@empty\else(\tikzchainprevious)%
edge[every join]#1(\tikzchaincurrent)\fi}}}
\makeatother
%
\tikzset{>=stealth',every on chain/.append style={join},
         every join/.style={->}}
\tikzstyle{labeled}=[execute at begin node=$\scriptstyle,
   execute at end node=$]
%
\ifnum\sigconf=0
    \usepackage[capitalise,nameinlink]{cleveref} %Incompatible with showonlyrefs
    \crefname{Game}{Game}{Games}
\fi
% \usepackage{autonum}%must be loaded after cleveref. Sometimes causes bugs. The alternative is incomaptible with cleveref:
 %\usepackage{mathtools} \mathtoolsset{showonlyrefs} %the mathtools way does not work nicely with sigconf. I *think* aotunum works in all cases. In any case, showonlyrefs does not work with cleveref.
 
 
%Due to incompatibility between cryptocode and autonum, the following hack is needed. https://tex.stackexchange.com/questions/522666/incompatibility-between-cryptocode-and-autonum:
\expandafter\let\expandafter\savedflalignstar\csname flalign*\endcsname
\expandafter\let\expandafter\savedendflalignstar\csname endflalign*\endcsname
\AtBeginDocument{%
  \expandafter\let\csname flalign*\endcsname\savedflalignstar
  \expandafter\let\csname endflalign*\endcsname\savedendflalignstar
}
 
 %Another compatability error here, I prefer to avoid autonum for now
\ifnum\sigconf=0
    \newtheorem{theorem}{Theorem} 
    \newtheorem{lemma}{Lemma}
    \newtheorem{corollary}{Corollary}
    \newtheorem{proposition}{Proposition}
    \newtheorem{definition}{Definition}
    \newtheorem{example}{Example}
    \newtheorem{conjecture}{Conjecture}
\fi 
  \newtheorem{claim}{Claim}
  \newtheorem{fact}{Fact}
  \newtheorem*{theorem*}{Theorem}
  \newtheorem*{lemma*}{Lemma}
  \newtheorem*{corollary*}{Corollary}
  \newtheorem*{proposition*}{Proposition}
  \newtheorem*{claim*}{Claim}
  
  \theoremstyle{definition}
  \newtheorem{openproblem}{Open Problem}
  \theoremstyle{remark}
  \newtheorem{remark}[theorem]{Remark}

  \theoremstyle{plain}
  \renewcommand{\qedsymbol}{$\square$}

\theoremstyle{plain}
\newcounter{Game} 
\setcounter{Game}{0}
\newenvironment{game}[1][htb]
    {
    \floatname{algorithm}{Game}% Update algorithm name
    \refstepcounter{Game}%to call the Game pointer. Currently the problem is that caption command by default calls the algorithm pointer. For the moment we need to use Game~~\ref{blah}
   \begin{algorithm}[#1]%
  }{\end{algorithm}}

% ---------------------------------------------------------------------------



%Abstract:
%\newcommand{\ab}[1]{#1} \newcommand{\fv}[1]{}

%Full version:
\newcommand{\ab}[1]{} \newcommand{\fv}[1]{#1} %%


\ifnum\masterthesis=1
    \usepackage{setspace}
    \onehalfspacing
    \usepackage{fancyhdr}
    \pagestyle{fancy}
    \fancyhf{}
    \renewcommand{\headrulewidth}{0pt}
    \renewcommand{\headheight}{14pt}
    \chead{\thepage}
    
    \newcommand{\longunderline}{\underline{\ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ }\ }
    
    \newenvironment{changemargin}[2]{%
        \begin{list}{}{%
        \setlength{\topsep}{0pt}%
        \setlength{\leftmargin}{#1}%
        \setlength{\rightmargin}{#2}%
        \setlength{\listparindent}{\parindent}%
        \setlength{\itemindent}{\parindent}%
        \setlength{\parsep}{\parskip}%
        }%
    \item[]}{\end{list}}
    
    \newcommand{\logoscale}{0.4}
\fi

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% end macros
